UniEP: Unified Expert-Parallel MoE MegaKernel for LLM Training

The exponential growth in Large Language Model (LLM) parameters has transformed model training into an increasingly resource-intensive endeavor. With the stagnation of Moore's Law and the widening disparity between computation throughput and communication bandwidth, expert parallelism (EP) has emerged as a critical strategy for scaling mixture-of-experts (MoE) models. However, despite numerous proposals for optimizing EP, ranging from communication compression to computation-communication overlap, adoption within production-grade frameworks like Megatron-LM remains conservative. Existing solutions often rely on ad-hoc, complex kernels that lack adaptability across diverse optimization configurations and frequently neglect numerical stability, failing to meet the strict precision requirements of large-scale training. In this paper, we introduce UniEP, a novel system that unifies diverse EP optimization strategies into a cohesive abstraction. UniEP fuses the MoE communication and computation into MegaKernels, effectively transforming complex architectural tuning into a unified parameter search space for automated adaptability. Crucially, UniEP incorporates a deterministic token ordering mechanism that guarantees numerical consistency with sequential execution, even under aggressive overlap schedules. We evaluate UniEP on GPU clusters equipped with NVIDIA Hopper GPUs. Our results demonstrate that UniEP achieves 1.03$\times$-1.38$\times$ speedups over state-of-the-art work, effectively mitigating communication bottlenecks while maintaining the rigorous accuracy standards required for production LLM training.

==> contents/3-overview.tex <==
\section{Overview of \ours{}}

==> contents/abstract.tex <==
\begin{abstract}
The exponential growth in Large Language Model (LLM) parameters has transformed model training into an increasingly resource-intensive endeavor. With the stagnation of Moore's Law and the widening disparity between computation throughput and communication bandwidth, expert parallelism (EP) has emerged as a critical strategy for scaling mixture-of-experts (MoE) models. However, despite numerous proposals for optimizing EP, ranging from communication compression to computation-communication overlap, adoption within production-grade frameworks like Megatron-LM remains conservative. Existing solutions often rely on ad-hoc, complex kernels that lack adaptability across diverse optimization configurations and frequently neglect numerical stability, failing to meet the strict precision requirements of large-scale training.

In this paper, we introduce \ours{}, a novel system that unifies diverse EP optimization strategies into a cohesive abstraction. \ours{} fuses the MoE communication and computation into {MegaKernels}, effectively transforming complex architectural tuning into a unified parameter search space for automated adaptability. Crucially, \ours{} incorporates a deterministic token ordering mechanism that guarantees numerical consistency with sequential execution, even under aggressive overlap schedules. We evaluate \ours{} on GPU clusters equipped with NVIDIA Hopper GPUs. Our results demonstrate that \ours{} achieves 1.03$\times$-1.38$\times$ speedups over state-of-the-art work, effectively mitigating communication bottlenecks while maintaining the rigorous accuracy standards required for production LLM training.
\end{abstract}

==> contents/history.tex <==
我觉得不用subsection，用textbf就行。好了，下面是我的内容，你要记得我们的abstract咋写的，保证intro和abstract一致性：

abstract:

The exponential growth in Large Language Model (LLM) parameters has transformed model training into an increasingly resource-intensive endeavor. With the stagnation of Moore's Law and the widening disparity between computation throughput and communication bandwidth, expert parallelism (EP) has emerged as a critical strategy for scaling mixture-of-experts (MoE) models. However, despite numerous proposals for optimizing EP, ranging from communication compression to computation-communication overlap, adoption within production-grade frameworks like Megatron-LM remains conservative. Existing solutions often rely on ad-hoc, complex kernels that lack adaptability across diverse optimization configurations and frequently neglect numerical stability, failing to meet the strict precision requirements of large-scale training.



In this paper, we introduce \ours{}, a novel system that unifies diverse EP optimization strategies into a cohesive abstraction. \ours{} fuses the entire MoE communication and computation workflow into a composable \emph{MegaKernel}, effectively transforming complex architectural tuning into a unified parameter search space for automated adaptability. Crucially, \ours{} incorporates a deterministic token ordering mechanism that guarantees numerical consistency with sequential execution, even under aggressive overlap schedules. We evaluate \ours{} on GPU clusters equipped with NVIDIA Hopper GPUs. Our results demonstrate that \ours{} achieves significant speedups over Megatron-LM, effectively mitigating communication bottlenecks while maintaining the rigorous accuracy standards required for production LLM training.

Motivation（主要说明优化MoE和EP的重要性和必要性）: 当前大模型主流架构是MoE（引用一些模型），世界一流的模型比如GPT-5，Gemini3Pro，DeepSeek-V3，Qwen3等都采用MoE架构，而且MoE专家数量越来越多，常见的专家数目在64-384。不仅仅是文本模型，现在的多模态模型也广泛使用MoE架构，比如Qwen-VL, DeepSeek-VL等。为了训练这些MoE模型，Expert Parallel训练方法被广泛使用，每个GPU获取一些专家，训练时GPU之间相互通信token。在实际模型训练中，MoE部分的开销（前向加反向）往往可以占据40%-70%（需要找一下文献佐证）。因此也有大量的工作优化MoE训练。

Limitation of state-of-the-art approaches: 对MoE的优化有很多方面，比如优化动态性（MegaBlocks），压缩模型大小（DeepSpeed-MoE），异构和分离式架构优化（HeterMoE），计算通信overlap（MegaScale-MoE，COMET），以及高性能MoE通信kernel（DeepEP, HybridEP）等。在主流的训练框架比如Megatron-LM中，集成了大量上述MoE优化技术，包括TransformerEngine以及MegaBlocks的高性能kernel和DeepEP的高性能通信kernel。

尽管这些工作很好地推动了MoE训练效率的提升，我们发现目前仍然有两点不足。

一方面，现有的工作将计算和通信作为分离的部分进行优化，然后再通过一些粗粒度的方法比如stream control的方式将计算和通信进行overlap，这一过程还需要host介入stream的同步，不同rank之间的进度不一致经常导致额外同步开销，优化效果往往是sub-optimal。而且在不同stream上切分microbatch也会造成训练精度的不稳定，特别是在反向传播时候对于weight的grad计算时候对token顺序非常敏感，两个microbatch之间的累加顺序无法保证。另一方面，现有工作无法统一通信原语。现在的训练框架仍然根据不同的模型参数，使用不同的通信primitive。比如当MoE中topk比较大时候，AllGather比AllToAll更节省通信量，反之则用AllToAll更合适，这就导致EP kernel开发和调优十分复杂，往往需要在大量可选的通信与计算kernel之间不断调整，既需要选原语，有需要选每个kernel的优化参数。为了解决这两个问题，我们提出了\ours{}。

Key insights and contributions: 我们关注在MoE EP训练的计算通信优化问题，并解决上述的两个问题。我们的insight有亮点：首先，在GPU上有办法可以不使用多stream就能完成计算通信overlap，而是使用SM（streaming multiprocessor）级别的控制，粒度更细，效果更好，也能避免切分batch带来的数值精度问题。其次，我们可以用统一的方式进行MoE EP计算和通信，避免依赖人工在不同的通信原语之间进行选择，而且可以统一自动调优整个MoE EP部分。

对于第一点，我们提出将MegaKernel技术应用在MoE训练中。以往的MegaKernel（引用Mirage, Triton-dist，HazyResearch）技术主要应用于推理，且总是把整个LLM融合到一个kernel里。我们则是首次把MegaKernel应用到训练，而且选择只融合MoE中的部分结构：dispatch+groupgemm和groupgemm+combine。在MegaKernel中，不同SM会承担不同的任务，有的SM负责通信，有的SM负责计算，通信和计算的SM之间存在数据依赖，则是通过额外的scoreboard记录依赖。我们的scoreboard可以达到token粒度，从而允许token级别的细粒度overlap。整个过程之需要一个stream，无需cpu介入，消除了额外同步开销，且可以大大提高SM的利用率，提高整体性能。

对于第二点，在我们的MegaKernel中，可以同时兼具AllGather和AllToAll的优点。我们提出了token remapping策略，可以做到避免重复token的通信，从而保证无论topk大或者小，通信量都和使用AllGather与AllToAll中最优的一致。另外，我们将MegaKernel中计算和通信的优化空间抽象为参数空间，允许MegaKernel无需编译就可以动态自适应不同的输入形状。这些优化参数构成的优化空间也很大，不能依赖人工选取，我们进一步提供了一个准确的硬件性能模型辅助寻找最优参数。

总结来说，我们的contribution主要是三点：

1. MoE训练的MegaKernel，实现了MegaKernel首次应用于训练，且可以在无cpu开销的情况下完成高效计算通信overlap和保持高精度数值

2. 通过token remapping技术和参数化技术，我们实现了对不同MoE workload的全自动调优和适配，避免人工复杂调优，实现易用性和高性能

3. 我们在实际的workload中进行大量测试，验证了\ours{}的性能和精度，也在128卡级别的训练任务中实际应用，明显提升性能

Experimental methodology and artifact availability: 我们在现代Nvidia Hopper GPU集群中进行测试，使用两种GPU规格，测试不同计算和带宽比例下的效果。我们对比的对象是权威的训练框架Megatron-LM中的MoE模块，其中集成了当前sota的kernel。我们测试的workload来自真实的LLM，包括DeepSeek, Qwen, Kimi等。我们还测试不同的microbatch和seqlen配置下的性能。最后，我们还在128卡级别进行端到端训练部署，验证精度和性能提升。我们的代码也将会开源。



我觉得你需要写大改双栏一页半的量



接下来是background，需要写大半页。

这一章我们主要介绍当前EP MoE的优化方式。

首先介绍整个MoE的训练结构，整体结构如图xx所示。在MoE前向传播中，首先需要计算专家的路由（routing），再根据路由信息计算每个专家收到的token数目，从而确定每个token通信发送的位置（每个token发送topk次，每次选不同的专家），这里每个token发送到哪个rank的哪个专家是确定的，但是发送到对应专家后，排列在对应专家收到的token的序号是有很多选择的。训练时候一般会选择一个稳定顺序（stable sorting），但是稳定顺序有很多选择，比如正序排列，倒序排列，或者别的确定性顺序，不同kernel实现不同，造成精度不一致。经过排序后，就会开始通信过程，这个过程一般叫dispatch，dispatch可以通过allgather所有token后scatter，也可以通过all2all直接完成。dispatch之后就是连续的groupgemm+swiglu激活+groupgemm，计算后的token最终被combine到每个rank结束MoE，combine的过程是把每个token的topk份结果从远端拷贝回来然后做加权累加。combine可以通过reduce-scatter后topk-reduce或者all2all+topk-reduce完成。

MoE的反向更为复杂，需要按照forward相反的顺序，对output grad进行dispatch，groupgemm+swiglu-backward+groupgemm+combine，这样可以计算出对于输入的grad，计算对weight的grad，则需要transposed groupgemm，transposed groupgemm和普通的groupgemm区别在于，普通的groupgemm在输入的spatial维度是切分group的，但是transposed groupgemm在累加维度切分group，因为它的累加维度正好对应microbatch和seqlen的维度。这一特性也导致如果在microbatch和seqlen维度切分了双batch，那么两个sub-batch计算weight的累加顺序就会发生变化，导致最后的结果精度发生变化。

其次，我们讲对MoE的主要优化手段。

首先是group gemm的优化。由于MoE通信后的token数目是动态的，groupgemm需要处理动态形状的输入。在MegaBlocks和vLLM中都有实现免padding的动态group gemm，这种groupgemm将每个专家需要计算的token按照固定大小分块（比如128个token一个tile），通过在groupgemm kernel内动态计算每个tile的offset来应对动态形状。这种groupgemm可以减少memory压力，同时性能可以做到理论性能的65%以上（在Hopper GPU上，大概是650TFLOPS以上），这种分块的设计也是后续overlap计算和通信的基础。

其次是对通信优化，COMET和DeepEP这种通信库基于NVSHMEM开发高性能通信算子，COMET使用AllGather，DeepEP则使用AllToAll。这些通信都需要额外的通信资源，比如DeepEP切分20个SM用于通信，相对应的计算资源就需要减少。

最后是overlap优化，对于MoE的计算通信overlap，COMET使用的是tile级别overlap，将AllGather和GroupGEMM发射在两个不同的stream上，两个stream之间通过global memory中的barrier进行通信，AllGather完成一个tile的通信，就会通知GroupGEMM进行计算。DeepEP则是使用双batch overlap，当一个stream上运行batch1的通信时，另一个stream上运行第二个batch的计算。可以看到，已有的做法都需要双stream，stream的控制不可避免会有cpu介入，这也是同步代价引入的地方。






现在开始写技术章节，技术章节我分两个section，第一个section写两页。内容如下：

section 3: Unified Overlapping MegaKernel

\ours{}首先不使用双batch overlap，也不使用双stream，而是使用一整个kernel融合计算和通信，在不同的SM上分配不同的任务，SM之间相互overlap。这样的MegaKernel设计比较复杂，我们将在这章讲解如何设计这样的MegaKernel。

\subsection{Dispatch+GroupGEMM MegaKernel Design}

在图~\ref{fig:moe_structure}里我们看到一个经常出现的pattern就是Dispatch+GroupGEMM，因此将这个pattern实现为一个MegaKernel既可以充分利用计算通信overlap的机会，也可以保证足够的模块化和可复用性。

首先，MegaKernel是persistent kernel，根据GPU的SM数量，我们只启动SM这么多个threadblock，每个threadblock作为一个worker，这样可以保证每个threadblock独占一个SM，更方便做SM之间的调度和协同。此外，有时需要做所有worker的同步，如果worker的数目超过了SM，可能造成死锁（等待的SM没有被实际调度到SM上）。

其次，在MegaKernel内，worker有三种角色：通信worker，负责发送token；计算worker，负责groupgemm计算；relay worker，负责统计到达的token情况并触发计算worker。下面我们详细介绍三种worker的设计。

\textbf{通信woker}。通信worker根据index compute的结果发送token。为了兼容不同的token顺序，从而满足和任意stable的baseline可以做到精度bitwise，通信worker需要按照index compute计算的顺序计算token实际发送的顺序。index compute的结果是local的，它只计算了当前rank的token应该发送到每个expert的具体位置，这样的index layout是token_id -> (expert_id, id_in_expert)。而通信worker要根据所有rank的这个信息构造出的映射token_id->(rank_id, expert_id_within_rank, id_in_expert_after_dispatch)来发送token，这个映射具体构造的算法如下：

（写一个algorithm，注意需要双栏的单侧能放下，变量名字可以适当调整）

IN: selected_experts: 每个rank的topk id信息

IN: local_token_mapping: 任意local stable sorting, shape[tokens_per_rank, topk]

OUT: global_token_mapping: token_id到rank_id, expert_in_rank_id, id_in_expert

expert_counts = bincount(selected_experts, num_bins=num_experts)

expert_offs = expert_counts.cumsum(dim=-1)

all_expert_counts = allgather(expert_counts) # shape [world_size, num_experts]

all_offs = all_expert_counts.view(world_size, -1, world_size).permute(2, 1, 0).view(world_size, -1).cumsum(dim=-1).view(world_size, -1, world_size) # 计算每个expert收到的token的offset

for rank in range(world_size):

  for t in range(num_tokens_per_rank):

    for j in range(topk):

      to_expert = selected_experts[t, j]

      to_rank = to_expert // experts_per_rank

      expert_id_in_rank = to_expert % experts_per_rank

      offs = all_offs[to_rank, expert_id_in_rank, rank]

      local_idx = local_token_mapping[t, j]

      final_idx = local_idx - expert_offs[to_expert] + offs

      global_token_mapping[t, j] = final_idx

这个算法可以接受任意的local_token_mapping，最终得到一致的global token mapping顺序，从而保证了计算的bitwise。

基于token mapping结果，通信worker中的每个warp负责发送一个token，一个warp内的32个线程按照128bit的vector大小切分token，每次发送大小为128bit。每个通信worker的warp数目可以调整，从而可以控制通信的并行度。

\textbf{计算worker}：每个计算worker负责一个tile的group gemm计算。每个计算worker首先需要确定当前的tile依赖的token是否都达到，当确认这个tile所有的token都被通信worker发送到位之后，就会进行这个tile内的group gemm计算，具体的计算流程按照vLLM和MegaBlocks的技术，也是padding-free，动态计算ptr offset来根据token选择的专家load weight data，然后利用tensor core完成计算。

\textbf{relay worker}：每个relay worker负责监视一个tile的groupgemm需要的token是否都到达了，每次通信worker发送成功一个token时候，都会同时写一个信号，信号存放在global memory中，relay worker每次收到一个token都会将自己的计数器加一，等到计数器的值和tile size一致的时候，就会写一个信号给计算worker，通知这个tile的token全部到达。



上述worker之间通信的机制，是通过在global memory中由软件维护一个scoreboard，scoreboard的本质就是一个array，它的layout组织如下：[token_size | groupgemm tile size]，前一半用于通信worker写token到的信号，后半部分长度和groupgemm的tile数目相关，用来通知计算worker计算开始。因为这些数量都是动态，所以scoreboard的大小往往是按照最大值开辟的，因为token数量一般小于128K，groupgemm tile数量一般小于1K，整体的内存开销非常小（约1MB）。

worker的角色分配可以是动态的，也可以是静态的。静态方案相对不灵活，就是在kernel启动时候，人为固定每个SM的角色。静态方案的另一个弊端是难以控制不同SM的负载均衡，因为有的SM可能比较快结束，比如通信量比较小的时候，通信可以提前结束，但是计算还需要很久，当时静态分配给通信的worker无法用于计算，造成资源浪费。动态方案则可以解决这个问题。动态方案下，维护一个全局的counter，每个SM都会竞争counter，通过atomicAdd的方式增加counter并获取一个唯一的counter ID，这个counter ID就是它对应的任务ID，通过定义不同任务ID的范围，来确定每个SM当前的任务，比如可以规定前64个任务是通信，之后的8192个任务是计算。这个任务的定义可以在kernel launch时候根据problem size动态设置。当一个SM完成了当前任务，就会再次竞争任务ID，直到没有更多需要做的任务为止。通过这种方式，我们可以实现负载均衡。

我们用图xx来辅助理解上述workflow，图xx中展示了三个不同角色的worker。我们用横轴表示时间，最开始所有的SM竞争counter，获取自己的task ID，然后分工进行通信与计算，最开始计算需要等待通信，所以它们有一段等待的空白，而通信worker一开始就可以做通信，并不断更新scoreboard，relay worker则不断查看scoreboard直到可以通知计算worker开始计算。一段时间后，就会有计算worker启动开始计算，此时计算、通信、relay都是并行进行的。当通信结束时，SM可以立即获取新的计算任务，转换为计算worker，并进行计算。

\textbf{relay worker的作用与通信量节约的优化}
这里我们设计的relay worker，其实可以省略，因为通信worker可以直接写信号给计算worker。但是我们仍然使用relay worker这一个中间件，是因为可以使用通信量节约的优化。每个token在被复制topk份发给不同的expert的时候，是有一定概率会发送到同一个rank的不同expert上，这就带来了通信量减少的机会。对于发送到同一个rank不同expert的token，我们只需要发送一次，然后通过relay worker来在目标rank进行一次内存拷贝实现多份复制。通信走的是NVLink带宽，而内存拷贝用的是HBM带宽，后者是前者的10x以上。所以可以带来额外的加速。我们还可以从理论上计算着一优化带来的通信量减少的期望值，假设topk=8而且每个token发送到每个expert的概率均等：
token只发送到X张卡	节约的token发送数目	概率计算公式	计算结果
1	7	C(8,1)*1!*S(8,1)/8^8	0.00000048
2	6	C(8,2)*2!*S(8,2)/8^8	0.00042391
3	5	C(8,3)*5!*S(8,3)/8^8	0.01934624
4	4	C(8,4)*4!*S(8,4)/8^8	0.17033100
5	3	C(8,5)*5!*S(8,5)/8^8	0.42057037
6	2	C(8,6)*6!*S(8,6)/8^8	0.31963348
7	1	C(8,7)*7!*S(8,7)/8^8	0.06729126
8	0	C(8,8)*8!*S(8,8)/8^8	0.00240326
期望计算结果是每个token可以少发送2.75次，也就是减少了2.75/8约为34\%的通信量。


\subsection{GroupGEMM+Combine MegaKernel Design}
类似的，我们可以设计GroupGEMM+Combine的MegaKernel，避免重复，我们快速地介绍这个MegaKernel的设计，其中使用的技术都在前述Dispatch+GroupGEMM里介绍了。我们这次也是分三个角色：计算worker, 通信worker, reduce worker。计算worker计算GroupGEMM，每次完成一个tile都会写一个信号给通信worker。通信worker收到信号之后就会将这个tile里的token写到远端，并通过写远端的scoreboard通知远端的reduce worker。远端的reduce worker则是不断扫描自己的scoreboard，发现某个token的topk个副本都到达后，就可以把它们加权求和起来得到结果。注意这里一定要等到所有的topk个副本都到达，而不能为了介于通信量提前进行reduce，否则会破坏累加顺序从而破坏精度。
与Dispatch+GroupGEMM一样，我们也采用动态分配角色的方式控制SM的行为，从而达到负载均衡。


下面开始技术章节第二部分。

section{Optimization Space and AutoTuning}

这一章节，基于我们的MegaKernel，继续介绍调优技术。通过MegaKernel设计，我们可以通过high-level调控一些参数就控制通信行为。我们还为更好的计算通信overlap可以调整token通信的先后优先级。最后，我们把资源划分（SM数量和warp数量）都用统一的参数模板表示，并设计一个精准的性能模型帮助寻找最优参数。

\subsection{通信性能的调优选项}


我们对Dispatch+GroupGEMM的优化参数集中为三个参数：每个Worker拥有的warp数量，通信Worker的数量，Relay Worker的数量。我们一一介绍这三个参数，首先是warp数量。通信和Relay Worker的warp数量可选范围是8，16，32。因为MegaKernel中所有Worker的warp数量是一致的，一般来说计算Worker只需要8个warp就能充分利用Tensor Core资源，多余的warp可能造成warp scheduler过度繁忙从而造成GPU运行时候过热而降频；而对于通信Worker，warp越多，并行度越高，越容易打满带宽。这就造成了一个trade-off：为了通信效果好，需要选择多的warp，但是为了计算不降频，希望warp能少一些。
其次是通信Worker的数量，也就是通信task的数量定义。如果通信Worker过多，超过了GPU拥有的SM数量，那么最开始所有的SM都忙于通信，没有和计算overlap的机会。所以通信Worker一半设置少于SM数量。通信Worker数量也不能过少，不然并行度不足导致通信bound，整体的性能就会下降。所以通信Worker的数量是一个在[1,num\_sm)之间调优的参数，需要根据problem size动态调整，当计算部分任务比较重的时候，少分配一点通信Worker，当计算比较轻量级时候，多分配一些通信Worker。

最后是Relay Worker的数量，EP中的AllGather是在每个token被topk份复制之前进行的，把所有Rank的token全都gather起来，然后再根据topk ID的选择进行GroupGEMM，这个过程可以避免topk份复制造成的膨胀，可以节约通信量，通信量就是全部token的大小。而EP中的AllToAll对于每个目标Rank只传输它需要的token，但是传输是被膨胀topk倍的，所以通信量是每个Rank原本有的token量乘以topk。写出来公式就是：AllGather通信量：$W \times S \times token\_bytes$，其中W是world\_size，S是每个Rank的seqence length乘以micro batch size，token\_bytes是每个token的大小。AllToAll的通信量是$S \times topk \times token\_bytes$。在前面的Section~\ref{sec:design}我们介绍过我们可以通过Relay Worker实现通信量优化，期望上可以将通信量减少到$S \times 5.25 \times token\_bytes$。这一通信量压缩并非没有代价，我们需要分配足够的SM资源给Relay Worker。Relay Worker需要有和通信Worker相匹配的SM才能保证及时处理scoreboard更新从而及时触发计算Worker，否则整个kernel会bound在等待信号。但是Relay Worker的数量和通信Worker数量之和不能超过GPU的总SM数量，否则就会有风险让有的Relay Worker没有被调度上来，整个kernel进入死锁。所以它的范围一般是$[1, num\_sm - comm\_worker\_sm]$。

类似地，GroupGEMM+Combine也有三个优化参数：每个Worker拥有的warp数量，通信Worker的数量，和Reduce Worker的数量。
这些参数的具体选择，不能依赖人工选择，否则优化空间过大，难以调优。我们后面会介绍我们的性能模型来自动选择最优参数。


\subsection{token发送优先级决定overlap效果}
在之前，我们讨论过为了保持bitwise精度而做的token mapping。基于这个mapping，我们可以进一步确定token传输的优先级。每个token发送的位置都是唯一确定的，精度也是由这个空间位置确定的，但是发送的先后关系还没有确定。当token数目很多，而通信Worker不足时候，必然要先选择一个token发送，然后再发送其他的。这个顺序则会影响overlap效果。如果先发送的token并非远端Rank当前活跃的计算Worker需要的，那远端的计算Worker就会一直等待自己需要的token，阻塞了其他原本可以工作的计算Worker被调度。所以我们需要约定一个顺序，让当前活跃的计算Worker与通信Worker之间通信的token是对齐的。为此，我们约定计算Worker总是从自己Rank上的第0个专家所需要的token开始计算。而通信Worker优先发送每个其他Rank的0号专家的token，然后是1号专家的token，以此类推。这一优先级排序是现在通信Worker中，Worker维护一个array，这个array被按照专家顺序排列（因为专家之间的offset可以通过cumsum计算，所以这一排序在专家之间是并行的，不会造成通信Worker变慢），然后按照排序后的token优先级进行发送。

\subsection{性能模型与调优}
根据上述内容，我们的优化空间主要由六个参数组成，计作（w_disp, N_disp, N_relay, w_comb, N_comb, N_red）。我们在table~\ref{table:notation}中列出了相关的symbol。我们设计了一个性能模型和调优算法求解最优的参数。除了这六个符号，我们还在table里列出了性能模型需要的其他symbol，包含硬件配置，输入MoE规模，以及辅助的变量等。

具体的性能模型在给定问题规模P,硬件参数H，搜索空间S之后，就会遍历所有的参数组合，然后预测每个参数对应的性能，最终选择性能最好的（延迟最低的）。这一过程在算法~\ref{algo:perf_model}中展示。整体延迟由三部分组成（line 26），分别是Dispatch+GroupGEMM延迟，SwiGLU延迟，和GroupGEMM+Combine延迟。其中SwiGLU是memory bound的kernel，延迟计算最为简单（line 5）。对于Dispatch+GroupGEMM，需要首先计算GroupGEMM自身每个tile的延迟，以及Dispatch每个Worker的延迟，然后再将二者的延迟overlap起来（line 10-14），这个计算过程需要根据二者分配到的SM数目和warp数目计算分配到的硬件性能，我们在后面详细解释这里用到的CalcDispLat和CalcCompLat函数。类似的，对于Combine，也有两个函数分别计算Combine通信的延迟和Combine时候的GroupGEMM的延迟（line 17-18），这里用到的函数CalcCombLat也在后续介绍。注意GroupGEMM+Combine还有一个尾部的topk reudce，这个也需要参与overlap计算的延迟中（line 22-24）。下面，我们基于Table~\ref{tab:notation}里的符号介绍用到的几个重要函数：

（把下面的内容串通连贯起来，要和symtable和算法对应好，符号要一致）

\begin{table}[t]
\centering
\caption{Summary of Notations and Symbols}
\label{tab:notation}
\resizebox{\linewidth}{!}{% 自适应调整表格宽度以适应单栏
\begin{tabular}{l l}
\toprule
\textbf{Symbol} & \textbf{Description} \\
\midrule
\multicolumn{2}{c}{\textit{Hardware Specifications ($H$)}} \\
\midrule
$N_{SM}$ & Total number of Streaming Multiprocessors \\
$\mathcal{P}_{peak}$ & Peak compute performance (TFLOPS) \\
$\beta_{HBM}$ & Peak HBM bandwidth (GB/s) \\
$\beta_{NVL}$ & Peak NVLink bandwidth (GB/s) \\
$W_{sat}$ & Number of warps to saturate bandwidth (e.g., 1024) \\
$\tau_{sync}$ & Synchronization overhead between kernels ($\approx 2\mu s$) \\
\midrule
\multicolumn{2}{c}{\textit{Problem \& Constant Configs ($P$)}} \\
\midrule
$B_M, B_N$ & Block dimensions for GroupGEMM (e.g., 128, 256) \\
$\mu$ & GroupGEMM Model FLOPs Utilization (MFU) \\
$H_{dim}$ & Model Hidden Dimension \\
$H_{inter}$ & MoE Intermediate Dimension \\
$N_{tok}$ & Number of tokens per rank \\
$S_{tok}$ & Size of a single token in bytes (e.g., hidden\_size $\times 2$) \\
$V_{nvl}, V_{hbm}$ & Total data volume transmitted via NVLink/HBM \\
\midrule
\multicolumn{2}{c}{\textit{Optimization Variables ($C \in \mathcal{S}$)}} \\
\midrule
$w_{disp}$ & Number of warps allocated for Dispatch MegaKernel\\
$w_{comb}$ & Number of warps allocated for Dispatch MegaKernel\\
$N_{disp}$ & Number of SMs allocated for Dispatch Comm Worker \\
$N_{comb}$ & Number of SMs allocated for Combine Comm Worker \\
$N_{relay}$ & Number of Realy Workers in Dispatch\\
$N_{red}$ & Number of Reduce Workers in Combine \\
\midrule
\multicolumn{2}{c}{\textit{Latency \& Cost Model Variables}} \\
\midrule
$t_{up}, t_{down}$ & Execution time of a single Up/Down GEMM block \\
$L_{disp}$ & Latency of the Dispatch communication phase \\
$L_{comb}$ & Latency of the Combine communication phase \\
$L_{swiglu}$ & Latency of the element-wise SwiGLU kernel \\
$W_{gap}$ & Workload gap between GEMM and Combine phases \\
$W_{rem}$ & Remaining reduce workload that cannot be overlapped \\
$\mathcal{B}(n, \beta)$ & Effective bandwidth function given $n$ SMs \\
\bottomrule
\end{tabular}
}
\end{table}

\begin{algorithm}[t]
\caption{Performance Model \& Config Search}
\label{algo:perf_model}
\begin{algorithmic}[1]
\Require Problem $P$, Hardware $H$, Config Space $\mathcal{S}$
\Ensure Optimal Config $C^*$, Min Latency $L_{min}$

\State $L_{min} \gets \infty$; $C^* \gets \emptyset$
\ForAll{$C \in \mathcal{S}$}
    \State \Comment{\textbf{1. Basic Op Latency}}
    \State $t_{up}, t_{down} \gets \text{CalcGEMMBlockTime}(H, P)$
    \State $L_{swiglu} \gets \text{CalcSwigluTime}(P, H)$
    
    \State \Comment{\textbf{2. Stage 1: Dispatch + Up/Gate Overlap}}
    \State $N_{gemm1} \gets H.N_{sm} - C.N_{disp}$
    \State $L_{disp} \gets \text{CalcDispLat}(P, H, C.N_{disp}, C.N_{tail})$
    \State $L_{up} \gets \text{CalcCompLat}(P, t_{up}, N_{gemm1})$
    
    \If{$L_{up} > L_{disp}$}
        \State $L_{S1} \gets L_{disp} + (L_{up} - L_{disp}) \times \frac{H.N_{sm}}{N_{gemm1}}$
    \Else
        \State $L_{S1} \gets L_{disp} + t_{up}$
    \EndIf

    \State \Comment{\textbf{3. Stage 2: Down + Combine Overlap}}
    \State $N_{gemm2} \gets H.N_{sm} - C.N_{comb}$
    \State $L_{comb}, t_{red} \gets \text{CalcCombLat}(P, H, C.N_{comb})$
    \State $L_{down} \gets \text{CalcCompLat}(P, t_{down}, N_{gemm2})$
    
    \State \Comment{Estimate Reduce overlap (filling the gap)}
    \State $L_{base} \gets \max(L_{down}, L_{comb})$
    \State $W_{gap} \gets |L_{down} - L_{comb}| \times N_{gemm2}$ \Comment{Available slots}
    \State $W_{red} \gets C.N_{red} \times t_{red}$ \Comment{Total reduce work}
    \State $W_{rem} \gets \max(0, W_{red} - W_{gap})$
    \State $L_{S2} \gets L_{base} + W_{rem} / H.N_{sm}$

    \State \Comment{\textbf{4. Update Optimal}}
    \State $L_{total} \gets L_{S1} + L_{S2} + L_{swiglu}$
    \If{$L_{total} < L_{min}$}
        \State $L_{min} \gets L_{total}$; $C^* \gets C$
    \EndIf
\EndFor
\State \Return $C^*, L_{min}$
\end{algorithmic}
\end{algorithm}

\paragraph{Effective Bandwidth.} 
First, we define the effective bandwidth function $\mathcal{B}(n, \beta)$ given $n$ active SMs and peak bandwidth $\beta$ (either $\beta_{NVL}$ or $\beta_{HBM}$). Let $w$ be the number of warps per SM and $W_{sat}$ be the saturation threshold (empirically $32 \times 32$ warps). The available bandwidth is limited by either the hardware peak or the number of active warps:
\begin{equation}
    \mathcal{B}(n, \beta) = \min\left( n \cdot w \cdot \frac{\beta}{W_{sat}}, \beta \right)
\end{equation}

\paragraph{GEMM Block Latency (\texttt{CalcGEMMBlockTime}).}
The execution time of a single GroupGEMM tile depends on the FLOPs count and the effective throughput. Let $B_M, B_N$ be the block size, $K$ be the reduction dimension ($H$ for Up/Gate, $H_{inter}$ for Down), and $\mu$ be the Model FLOPs Utilization (MFU).
\begin{equation}
    t_{gemm}(K) = \frac{2 \cdot B_M \cdot B_N \cdot K}{\mathcal{P}_{peak} \cdot (\mu / N_{SM})} + \tau_{sync}
\end{equation}
where $\mathcal{P}_{peak}$ is the GPU peak performance and $\tau_{sync}$ is the synchronization overhead (approx. $2\mu s$). Thus, $t_{up} = t_{gemm}(H_{dim})$ and $t_{down} = t_{gemm}(H_{inter})$.

\paragraph{SwiGLU Latency (\texttt{CalcSwigluTime}).}
SwiGLU is an element-wise operation bound by HBM bandwidth. For $N_{tok}$ tokens with size $S_{tok}$:
\begin{equation}
    L_{swiglu} = \frac{2 \cdot N_{tok} \cdot S_{tok}}{\beta_{HBM}}
\end{equation}

\paragraph{Dispatch Latency (\texttt{CalcDispLat}).}
The dispatch process involves moving tokens via NVLink (for remote experts) and HBM (for local experts). Let $V_{nvl}$ and $V_{hbm}$ be the total data volume for remote and local transmission respectively.
\begin{equation}
    L_{disp} = \frac{V_{nvl}}{\mathcal{B}(N_{disp}, \beta_{NVL})} + \frac{V_{hbm}}{\mathcal{B}(N_{disp}, \beta_{HBM})}
\end{equation}
Note that if tail SMs are used for broadcasting, their HBM contribution is calculated separately with $N_{relay}$ and added to the total.

\paragraph{Combine Latency (\texttt{CalcCombLat}).}
Similar to Dispatch, Combine involves gathering data via NVLink and performing reduction in HBM.
\begin{align}
    L_{comb\_scatter} &= \frac{V_{nvl}}{\mathcal{B}(N_{comb}, \beta_{NVL})} \\
    t_{red} &= \frac{V_{hbm\_total}}{\mathcal{B}(1, \beta_{HBM})} \quad (\text{latency per SM})
\end{align}
Here, $t_{red}$ represents the time for one SM to reduce its assigned portion of tokens.

\paragraph{Computation Latency (\texttt{CalcCompLat}).}
The total computation time for a stage is determined by the number of "waves" required to process all tiles on the allocated SMs. Let $N_{tiles}$ be the total number of GEMM blocks.
\begin{equation}
    L_{comp}(N_{sm}, t_{block}) = \left\lceil \frac{N_{tiles}}{N_{sm}} \right\rceil \cdot t_{block}
\end{equation}


下一章节讲实现。

\section{Implementation of \ours{}}

实现MegaKerenl需要大量的底层调优。如果从CUDA层面开始实现，工程量会非常大。为此，我们选择了一个更方便的框架Triton-distributed。我们利用Triton-distributed拓展的Triton语法完成MegaKernel的编程，并且把我们的perf model实现出来用于设置最优的调优参数。
整个MegaKernel部分的代码长度是21k行的Python code。这也体现了我们选择Triton-distributed的优势，如果用CUDA来实现，代码长度可能达到5-10倍的长度。
Triton-distributed为我们提供以下几个编程优势：
1. 原生的NVSHMEM支持，可以直接写分布式通信kernel
2. 信号管理，可以使用带有内存语义的load/store指令控制同步
3. warp级别的控制，Triton-distributed拓展了Triton的SPMD编程模型，打开了warp级别的控制，可以做warp id获取，warp级别sync，以及warp级别的memory copy等。

我们的Dispatch+GroupGEMM MegaKernel伪代码如下：

def dispatch_group_gemm(...):
   sm_id = tl.program_id(0)
   task_id = tl.atomic_add(counter, 1)
   while task_id < valid_num_tasks:
     if get_task(task_id) == GroupGEMM:
        # do group gemm tile
     elif get_task(task_id) == Dispatch:
        # do dispatch
     elif get_task(task_id) == Relay:
        # do relay
     task_id = tl.atomic_add(counter, 1)

类似地我们实现GroupGEMM+Combine MegaKernel。
对于通信Worker，我们的通信是通过NVSHMEM原语实现的。Triton-distributed内部支持全部的NVSHMEM原语，我们选择putmem_warp作为主要的通信原语，因为putmem比getmem能获得的带宽更高，而且warp级别的控制符合我们的需求。对于信号控制，则使用Triton-distirbuted提供的st_release和ld_acquire指令，保证了内存一致性。
对于计算Worker，我们直接用dot和load等Triton high-level原语实现。虽然我们没有用TMA，但是对于GroupGEMM这种workload来说，已经可以取得和CUTLASS相当的性能。对于tile size 128x256x64来说，每个tile的运行时间是22us左右，已经将Tensor Core利用率打到60%-70%。
对于Relay Worker和Reduce Worker，我们也是用的warp级别控制，每个warp负责一个token，从而达到高并行度。
实现好MegaKernel之后，我们按照图~\ref{fig:moe_structure}实现了forward和backward，并接入到端到端的模型训练任务中。

对于performance model，我们用Python和C++各实现了一版，整个搜索空间的大小约为1e5，Python版本顺序遍历搜索一次需要100s左右，这在真实训练场景难以接受。我们用C++和OpenMP实现并行版本，优化到144ms左右的速度。为了复用调优结果，我们将输入的seqlen进行分桶，以4k为单位，也就是说我们调优时候传入给perf model的N_{tok}都是4k对齐的。这样调优只需要在训练中N_{tok}越过桶边界进行一次即可，之后可以一直复用调优后的config。


现在我们写evaluation
\section{Evaluation}

\subsection{Evaluation Setup}
我们的硬件集群环境是两台搭载NVLink的Hopper GPU集群。cluster 1有8个GPU，每个GPU有80GB HBM，NVLink的单向带宽有200GB/s，另一个cluster 2有8个GPU，每个GPU有96GB HBM，NVLink的单向带宽有400GB/s。我们在Table~\ref{xxx}里列出两个集群的配置（列一个小表，列出来GPU数目，HMB大小，HBM带宽，NVLink带宽，每个GPU峰值BF16算力）。我们测试的MoE配置来自真实的网络，包括DeepSeek系列模型, Qwen系列模型，和Kimi系列模型。我们在Table~\ref{xxx}展示每个配置对应的模型名字和详细参数（列一个表，列需要包括代称（MoE1-12），模型名字（名字在下面的shapes里，按顺序），H_dim, H_inter, N experts, topk，12行）。我们还测试每个配置下不同的seqlen的性能，包括8k, 32k, 128k。最后，我们会测试端到端128卡训练的收益。我们性能对比的对象有两个：不做overlap优化，只做通信优化的baseline，这个baseline我们称为Serial。Serial里我们用DeepEP做EP通信，GroupGEMM用TransformerEngine的kernel，不做任何的overlap。另一个对比对象是COMET。COMET是目前state-of-the-art EP overlap训练解决方案。它通过把NVLink通信和GroupGEMM计算在两个stream上做overlap的方式提高训练性能，并且在企业级训练任务中验证过。

\subsection{Optimization Configs}
我们首先展示performance model预测的优化配置的选择，因为篇幅有限，我们只展示cluster 1上seqlen 32k对应的配置。（这里列一个表，下面的数据分别是对应MoE代号（1-12），然后config tuple里的数字的意思是N_disp, N_comb, N_relay, N_red, warps）。我们的performance model预测的准确率较高，为了做验证，我们对Kimi-K2, Qwen3-235B, Qwen3-30B的全部优化配置，列出最优配置和我们model找到的配置对应的性能差距（上万个配置，需要几小时全部测试完毕），最终发现我们找到的优化配置（注意我们的model只需要~140ms找到）和实际最优的配置在绝对性能误差（ms）在0.5%-6.5%之间。我们在图~\ref{xxx}中展示了误差，这表明我们的performance model非常准确。
1408,2048,6,32768,64,12501.42247984762,(12, 20, 5, 0, 32)
896,1280,6,32768,64,5494.032164899129,(16, 28, 1, 0, 32)
1408,2048,6,32768,64,12503.147071390476,(12, 20, 5, 0, 32)
1536,5120,6,32768,160,34385.52577662338,(12, 20, 5, 0, 32)
2048,7168,8,32768,256,80846.641024,(8, 16, 1, 0, 32)
768,2048,8,32768,128,10414.644400761907,(16, 28, 5, 0, 32)
1536,4096,8,32768,128,36031.94152184243,(12, 20, 5, 0, 32)
2560,6144,8,32768,160,83920.8872437551,(8, 12, 1, 0, 32)
512,2048,10,32768,512,10038.046908672139,(20, 32, 5, 0, 32)
384,1024,6,32768,128,2556.28036555634,(28, 40, 5, 0, 32)
2048,7168,8,32768,384,83716.05753173333,(8, 16, 1, 0, 32)
1024,2304,8,32768,256,15216.17572595023,(16, 24, 1, 0, 32)

_shapes = [
    MoEShape(ffn_dim=1408, hidden_dim=2048, topk=6, ntotal_tokens=1024 * 8, num_experts=64), # DeepSeek-MoE-16B
    MoEShape(ffn_dim=896, hidden_dim=1280, topk=6, ntotal_tokens=1024 * 8, num_experts=64), # DeepSeek-OCR-2
    MoEShape(ffn_dim=1408, hidden_dim=2048, topk=6, ntotal_tokens=1024 * 8, num_experts=64), # DeepSeek-V2-Lite
    MoEShape(ffn_dim=1536, hidden_dim=5120, topk=6, ntotal_tokens=1024 * 8, num_experts=160), # DeepSeek-V2-Chat
    MoEShape(ffn_dim=2048, hidden_dim=7168, topk=8, ntotal_tokens=1024 * 8, num_experts=256), # DeepSeek-R1
    MoEShape(ffn_dim=768, hidden_dim=2048, topk=8, ntotal_tokens=1024 * 8, num_experts=128), # Qwen3-30B-A3B
    MoEShape(ffn_dim=1536, hidden_dim=4096, topk=8, ntotal_tokens=1024 * 8, num_experts=128), # Qwen3-235B-A22B
    MoEShape(ffn_dim=2560, hidden_dim=6144, topk=8, ntotal_tokens=1024 * 8, num_experts=160), # Qwen3-Coder-480B-A35B
    MoEShape(ffn_dim=512, hidden_dim=2048, topk=10, ntotal_tokens=1024 * 8, num_experts=512), # Qwen3-Next-80B-A3B
    MoEShape(ffn_dim=384, hidden_dim=1024, topk=6, ntotal_tokens=1024 * 8, num_experts=128), # Qwen3-Omni-30B-A3B
    MoEShape(ffn_dim=2048, hidden_dim=7168, topk=8, ntotal_tokens=1024 * 8, num_experts=384), # Kimi-K2
    MoEShape(ffn_dim=1024, hidden_dim=2304, topk=8, ntotal_tokens=1024 * 8, num_experts=256), # Kimi-Linear-48B-A3B
]

\subsection{对比kernel级别的性能}
首先我们对比Dispatch+GroupGEMM和GroupGEMM+Combine的性能。设置的seqlen是8k和32k（每个rank 1k和4k token）。我们在图~\ref{xxx}展示在两个cluster的性能。可以看到，对于Dispatch+GroupGEMM，在cluster 1上，8k seqlen下，\ours{}相比Serial的geometric mean加速是18.40x，对COMET的geometric mean加速是1.32x，32k seqlen下，我们没展示MoE8和MoE11，因为这些配置会out of memory，\ours{}相比Serial的geometric mean加速是11.20x，相对COMET的加速是1.30x。 在cluster 2上，对于8k seqlen，\ours{}可以取得相比Serial geometric mean 7.44x的加速，相比COMET，geometric mean 加速则是1.57x。对于32k seqlen，\ours{}相比Serial的geometric mean 加速比是3.57x，相比COMET geometric mean加速比是1.45x。对于GroupGEMM+Combine，cluster 1，相对Serial，在8k和32k seqlen下的平均加速是11.56x和8.23x，相对COMET的平均加速是1.31x和1.87x。在cluster 2，相对Serial，8k和32k seqlen平均加速是6.38x和2.58x，相对COMET加速则是1.21x和1.07x。

Serial的性能明显弱于COMET和\ours{}，即使Serial用了最好的通信kernel DeepEP，性能也非常差。我们发现DeepEP的dispatch时间明显长于combine时间，因为dispatch时候需要计算一些metadata留作给combine用，这部分开销是融合在通信kernel里的，不容易剥离。因此对比combine的性能更准确一些。单独看通信性能，DeepEP已经打满了NVLink带宽，但是计算部分的GroupGEMM使用的方法是每个专家调用一次GEMM，这样就需要不断从GPU拿shape信息回到CPU，造成太多不必要的sync，从而大幅降低性能。这种做法只有在计算量足够大，能让sync overhead不太重要的时候，才达到很好的效果。而相对COMET来说，我们的dispatch+GroupGEMM加速比combine明显，因为我们在dispatch会有利用relay worker做的通信量减少的优化。通过对比profiling trace，我们发现COMET还有性能损失是在于通信stream和计算stream之间kernel launch不对齐，造成额外的空泡，如果能消除这些空泡，COMET应该能取得一样好的性能。\ours{}由于MegaKernel之需要一个stream，就可以避免这个问题。

对比两种不同的cluster，我们也能发现，对于带宽较低的场景，比如cluster 1，overlap的收益更高，这是因为MoE此时是通信bound，能掩藏越多的通信开销，整体的加速就越明显。对于带宽较高的cluster 2，虽然收益降低了，但是仍然能带来加速，主要的收益则是来源于对不必要的同步开销的减少，这都依赖\ours{}细粒度调度和优化。

\subsection{对比Layer级别的性能}
我们继续对比MoE整个forward和backward性能。这部分计算里我们不计入gating（routing）的时间，虽然这部分时间也比较短，但是不在我们的优化范围内。实验结果在图~\ref{xxx}中展示。对于cluster 1，8k seqlen下，我们forward对于Serial的平均加速是11.98倍，backward则是4.00倍；对COMET的forward加速是1.08倍，backward是1.03倍。对于32k seqlen，forward对于Serial的平均加速是10.21倍，backward是4.12倍；对COMET的forward平均加速是1.22倍，backward平均加速1.18倍。

可以观测到在cluster 1我们的seqlen越长，相对COMET的收益越明显。这是因为token增多，通信中省掉不用发送的token的数量也会增加，但是在cluster 2就不一样，结论是相反的。因为cluster 2带宽比较高，节约通信收益不大。8k seqlen下，相对Serial的forward加速是4.17倍，backward加速是1.34倍；相对COMET forward加速是1.26倍，backward加速是1.17倍。在32k seqlen时候，forward相对Serial的加速是2.67x, backward是1.12x。相对COMET forward是1.19倍，backward是1.09倍。

\subsection{长文场景下的效果}
为了测试长序列的效果，我们还做了128k seqlen的实验。在cluster 1上，我们forward比Serial快6.90倍，比COMET快1.28倍；backward比Serial快4.12倍，比COMET快1.08倍。在cluster2， forward比Serial快2.38倍，比COMET快1.13倍；backward比Serial快1.01倍，比COMET快1.06倍。我们在图~\ref{xxx}中展示了对比，我们没有展示MoE5,MoE8,MoE11，因为这些配置在长文时候会out of memory。可以发现对于长文和高带宽场景，相比Serial的性能加速已经不明显，此时Serial的计算量足够大，额外sync的overhead已经不是bottleneck，我们仅有的收益都来自overlap，但是通信本身已经足够快，因此收益也并不像之前那样极为明显。尽管如此，我们仍然还是能拿到10%以上的收益，这对于训练来说意义也非常大，因为训练的卡量可以非常大，mfu一点点的提升也意味着巨大的cost节约。

\subsection{端到端训练效果}
我们实际将\ours{}用于内部训练，在MoE模型128卡训练任务中（使用16台cluster 1），seqlen达到512k，我们将吞吐从127B tokens/day提升到138B tokens/day，性能提高1.09倍。这也符合我们对于MoE单独测试的结果预期。更重要的是，我们的方式精度和串行执行完全bitwise，这对于训练来说异常重要。





接下来，我们写related work

\section{Related Work}
\ours{}主要受到三类工作的启发：高性能计算和通信Kernel工作，计算通信overlap工作，以及训练推理框架工作。

\subsection{高性能Kernel}
高性能Kernel开发主要有两种趋势：基于底层编程模型比如CUDA开发的kernel和基于high-level编程模型比如Triton, TileLang，CuTeDSL, CuTile等开发的。

\textbf{Expert-tuned High-performance Libraries}. 这类工作的代表有CuBLAS, CuDNN, CUTLASS/CuTe, FlashAttention, FlashInfer, DeepGEMM, NCCL, DeepEP等。他们通过CUDA编程，精细化控制诸如TMA和Tensor Core这种硬件单元完成高效计算。其中单卡计算kernel库比如CuBLAS和CUTLASS提供大量高性能的矩阵乘法和GroupGEMM kernel。通信库比如NCCL实现了大量高性能通信原语，比如AllGather, AllToAll, ReduceScatter, AllReduce等。NCCL中的通信原语专注于tensor parallel和sequence parallel，对于MoE中需要的EP通信支持较差。为此，DeepEP被开发出来，通过IBRC和IBGDA等机制实现高性能分布式EP通信，基本上可以打满带宽。DeepEP底层也是使用NVSHMEM原语。NVSHMEM提供了大量的peer-to-peer device侧function，可以允许在写CUDA kernel时候从device侧发起通信而不经过host。

\textbf{编译器}。高性能的Tensor 编译器通过提供DSL方便用户写高性能kernel。编译器将常用优化和常用的模板代码转换为生成的代码，从而让用户关注于优化和算法表达本身。Halide和TVM都采用compute和schedule分离的DSL。Mojo基于MLIR提供了全新的编程语言，可以达到和CUDA kernel匹配的性能。Triton和TileLang都基于Tile级别的编程模型，对上层开发提供易用性同时提供了高性能。CuTile和CuTeDSL都是NVIDIA最新推出的编译器，可以在Python层面完成和CUDA开发同样的能力。通信方面，也有编译器。MSCCL系列工作提出了通信的put/get等原语，基于NCCL封装了通信代码生成策略。

\subsection{计算通信Overlap工作}
计算通信Overlap方法众多，基于多stream方法最为常见。以Centauri，Megatron-LM，TorchTitan等工作为代表的框架工作通过将计算和通信放在不同的stream，甚至会适当切分计算和通信，以实现相互overlap。但是这种方式一方面切小了算子，造成每个小kernel内的wave数之和大于原本的kernel wave数目，也就是所谓的quantization effect，这会导致计算效率降低。另外，两个stream之间的相互同步和kernel launch需要cpu介入，这会导致额外的开销。为了解决这一问题，CoCoNet, DistEinsum，FLUX, COMET, TileLink, Pallas, FlashOverlap等工作通过在kernel间相互通信信号的方式避免了多次kernel launch，他们在两个stream上分别放置两个kernel，一个负责计算，一个负责通信，每个tile完成时候，producer就会通过global memory给consumer发信号。这种方式避免了cpu launch kernel造成的rank间时序不同步，但是仍然依赖两个stream。另一些工作比如DeepSeek-V3则是使用DeepEP结合双batch进行overlap，尽管对于部分训练场景可以接受，但是对于其他训练场景比如FSDP训练，强行切分两个batch会导致精度受损，在实际训练中难以接受。相比他们，\ours{}则是在一个stream内完成了计算和通信的overlap，完全避免了cpu的介入，而且可以做更细粒度的优化，比如SM级别的调度。

\subsection{训练推理框架}
对于MoE有大量的训练推理优化工作。比如TransformerEngine提供了高性能的GroupGEMM，MegaBlocks提供了动态性的MoE实现，vLLM集成了高性能Triton版本的GroupGEMM，MoEBlaze实现了内存节约的MoE，HeterMoE在异构集群上优化MoE训练，DeepSpeed-MoE优化了模型大小和通信性能，MegaScale-MoE使用FLUX的overlap kernel掩藏通信开销。尽管众多的MoE优化被提出，在要求严格的训练场景中，能满足需求的MoE实现仍然较少，特别的，在Megatron-LM这类工业级框架中，overlap优化使用仍然非常局限。而\ours{}不仅完全使用了overlap优化，也可以满足工业级训练的要求。

==> sections/approach.tex <==
\section{Approach}

%\subsection{Hello World}

==> sections/experiments.tex <==
\section{Experiments}

%\subsection{Hello World}


\section{Conclusion}

==> sections/introduction.tex <==
\section{Introduction}

%\subsection{Hello World}

==> sections/relatedwork.tex <==
\section{Related Work}

%\subsection{Hello World}
